The AdS/CFT Correspondence and Light-Front QCD

We identify an invariant light-front coordinate $\zeta$ which allows the separation of the dynamics of quark and gluon binding from the kinematics of constituent spin and internal orbital angular momentum. The result is a single-variable light-front Schrodinger equation for QCD which determines the eigenspectrum and the light-front wavefunctions of hadrons for general spin and orbital angular momentum. This frame-independent light-front wave equation is equivalent to the equations of motion which describe the propagation of spin-$J$ modes on anti-de Sitter (AdS) space. Light-front holography is a remarkable feature of AdS/CFT: it allows hadronic amplitudes in the AdS fifth dimension to be mapped to frame-independent light-front wavefunctions of hadrons in physical space-time, thus providing a relativistic description of hadrons at the amplitude level. In principle, the model can be systematically improved by diagonalizing the full QCD light-front Hamiltonian on the AdS/QCD basis. Quark and gluon hadronization can be computed at the amplitude level by convoluting the off-shell $T$ matrix calculated from the QCD light-front Hamiltonian with the hadronic light-front wavefunctions. We also note the distinction between static observables such as the probability distributions computed from the square of the light-front wavefunctions versus dynamical observables such as the structure functions and the leading-twist single-spin asymmetries measured in deep inelastic scattering which include the effects of initial and final-state interactions.

==> debug_log_12731 <==

#####Fri Oct 10 08:50:47 2008#####
STARTED admin_hep-ph.gfdt.19143


#####Fri Oct 10 08:50:47 2008#####
------------------------------------------------------------------------------
\\
arXiv:0810.1875
From: Guy F. de T\'eramond <gdt@asterix.crnet.cr>
Date: Fri, 10 Oct 2008 02:45:58 GMT   (000kb)

Title: The AdS/CFT Correspondence and Light-Front QCD
Authors: Stanley J. Brodsky and Guy F. de Teramond
Categories: hep-ph
Comments: 12 pages, 4 figures. Presented by SJB at LIGHT CONE 2008:
  Relativistic Nuclear and Particle Physics
Report-no: SLAC-PUB-13428
License: http://arxiv.org/licenses/nonexclusive-distrib/1.0/
Policy: accept
Upload-archive: hep-ph
Upload-subject: hput admin_hep-ph.gfdt.19143 figscombine.pdf LFHolography.pdf
  StaticDynamic.pdf
archive: hep-ph
is-an-author: 1
\\
  We identify an invariant light-front coordinate $\zeta$ which allows the
separation of the dynamics of quark and gluon binding from the kinematics of
constituent spin and internal orbital angular momentum. The result is a
single-variable light-front Schrodinger equation for QCD which determines the
eigenspectrum and the light-front wavefunctions of hadrons for general spin and
orbital angular momentum. This frame-independent light-front wave equation is
equivalent to the equations of motion which describe the propagation of
spin-$J$ modes on anti-de Sitter (AdS) space. Light-front holography is a
remarkable feature of AdS/CFT: it allows hadronic amplitudes in the AdS fifth
dimension to be mapped to frame-independent light-front wavefunctions of
hadrons in physical space-time, thus providing a relativistic description of
hadrons at the amplitude level. In principle, the model can be systematically
improved by diagonalizing the full QCD light-front Hamiltonian on the AdS/QCD
basis. Quark and gluon hadronization can be computed at the amplitude level by
convoluting the off-shell $T$ matrix calculated from the QCD light-front
Hamiltonian with the hadronic light-front wavefunctions. We also note the
distinction between static observables such as the probability distributions
computed from the square of the light-front wavefunctions versus dynamical
observables such as the structure functions and the leading-twist single-spin
asymmetries measured in deep inelastic scattering which include the effects of
initial and final-state interactions.
\\


#warnings_now: ADMIN UPLOAD



#author_warnings_now: 
Author 1: Stanley J. Brodsky
Author 2: Guy F. de Teramond
-> Number of authors = 2



#####Fri Oct 10 08:50:47 2008#####
Finished unpacking (errors=)

#author_warnings_now: 
Author 1: Stanley J. Brodsky
Author 2: Guy F. de Teramond
-> Number of authors = 2

 9999151.tar: unpacked 5 files from tar file
 hep-ph.gfdt.19143.tar: unpacked 5 files from tar file


#####Fri Oct 10 08:50:47 2008#####
showtime: 0810.1875 being processed as test/9999151 -> /data/ftp/arxiv/papers/0810


#####Fri Oct 10 08:50:47 2008#####
packing to 0810.1875.tar.gz

#####Fri Oct 10 08:50:47 2008#####
running AutoTeX -p test/9999151 -d 0810.1875 at Fri Oct 10 08:50:47 2008

#####Fri Oct 10 08:50:48 2008#####
completed AutoTeX in 1s

#####Fri Oct 10 08:50:48 2008#####
Rejected after unpack_submission()... cleaning up

#warnings_now: ADMIN UPLOAD

Fri Oct 10 08:50:48 2008: AutoTeX took 1s


#####Fri Oct 10 08:50:48 2008#####
About to close and move this log to /u0/incoming/admin_hep-ph.gfdt.19143 which will then be moved to /u0/incoming/rejects


==> debug_log_13850 <==

#####Fri Oct 10 08:52:36 2008#####
STARTED admin_hep-ph.gfdt.19143


#####Fri Oct 10 08:52:36 2008#####
------------------------------------------------------------------------------
\\
arXiv:0810.1875
From: Guy F. de T\'eramond <gdt@asterix.crnet.cr>
Date: Fri, 10 Oct 2008 02:45:58 GMT   (000kb)

Title: The AdS/CFT Correspondence and Light-Front QCD
Authors: Stanley J. Brodsky and Guy F. de Teramond
Categories: hep-ph
Comments: 12 pages, 4 figures. Presented by SJB at LIGHT CONE 2008:
  Relativistic Nuclear and Particle Physics
Report-no: SLAC-PUB-13428
License: http://arxiv.org/licenses/nonexclusive-distrib/1.0/
Policy: accept
Upload-archive: hep-ph
Upload-subject: hput admin_hep-ph.gfdt.19143 figscombine.pdf LFHolography.pdf
  StaticDynamic.pdf
archive: hep-ph
is-an-author: 1
\\
  We identify an invariant light-front coordinate $\zeta$ which allows the
separation of the dynamics of quark and gluon binding from the kinematics of
constituent spin and internal orbital angular momentum. The result is a
single-variable light-front Schrodinger equation for QCD which determines the
eigenspectrum and the light-front wavefunctions of hadrons for general spin and
orbital angular momentum. This frame-independent light-front wave equation is
equivalent to the equations of motion which describe the propagation of
spin-$J$ modes on anti-de Sitter (AdS) space. Light-front holography is a
remarkable feature of AdS/CFT: it allows hadronic amplitudes in the AdS fifth
dimension to be mapped to frame-independent light-front wavefunctions of
hadrons in physical space-time, thus providing a relativistic description of
hadrons at the amplitude level. In principle, the model can be systematically
improved by diagonalizing the full QCD light-front Hamiltonian on the AdS/QCD
basis. Quark and gluon hadronization can be computed at the amplitude level by
convoluting the off-shell $T$ matrix calculated from the QCD light-front
Hamiltonian with the hadronic light-front wavefunctions. We also note the
distinction between static observables such as the probability distributions
computed from the square of the light-front wavefunctions versus dynamical
observables such as the structure functions and the leading-twist single-spin
asymmetries measured in deep inelastic scattering which include the effects of
initial and final-state interactions.
\\


#warnings_now: ADMIN UPLOAD



#author_warnings_now: 
Author 1: Stanley J. Brodsky
Author 2: Guy F. de Teramond
-> Number of authors = 2



#####Fri Oct 10 08:52:36 2008#####
Finished unpacking (errors=)

#author_warnings_now: 
Author 1: Stanley J. Brodsky
Author 2: Guy F. de Teramond
-> Number of authors = 2

 9999151.tar: unpacked 9 files from tar file
 hep-ph.gfdt.19143.tar: unpacked 5 files from tar file


#####Fri Oct 10 08:52:36 2008#####
showtime: 0810.1875 being processed as test/9999151 -> /data/ftp/arxiv/papers/0810


#####Fri Oct 10 08:52:36 2008#####
packing to 0810.1875.tar.gz

#####Fri Oct 10 08:52:36 2008#####
running AutoTeX -p test/9999151 -d 0810.1875 at Fri Oct 10 08:52:36 2008

#####Fri Oct 10 08:52:37 2008#####
completed AutoTeX in 1s

#####Fri Oct 10 08:52:37 2008#####
Rejected after unpack_submission()... cleaning up

#warnings_now: ADMIN UPLOAD

Fri Oct 10 08:52:37 2008: AutoTeX took 1s


#####Fri Oct 10 08:52:37 2008#####
About to close and move this log to /u0/incoming/admin_hep-ph.gfdt.19143 which will then be moved to /u0/incoming/rejects


==> debug_log_14712 <==

#####Fri Oct 10 08:53:33 2008#####
STARTED admin_hep-ph.gfdt.19143


#####Fri Oct 10 08:53:33 2008#####
------------------------------------------------------------------------------
\\
arXiv:0810.1876
From: Guy F. de T\'eramond <gdt@asterix.crnet.cr>
Date: Fri, 10 Oct 2008 02:45:58 GMT   (000kb)

Title: The AdS/CFT Correspondence and Light-Front QCD
Authors: Stanley J. Brodsky and Guy F. de Teramond
Categories: hep-ph
Comments: 12 pages, 4 figures. Presented by SJB at LIGHT CONE 2008:
  Relativistic Nuclear and Particle Physics
Report-no: SLAC-PUB-13428
License: http://arxiv.org/licenses/nonexclusive-distrib/1.0/
Policy: accept
Upload-archive: hep-ph
Upload-subject: hput admin_hep-ph.gfdt.19143 figscombine.pdf LFHolography.pdf
  StaticDynamic.pdf
archive: hep-ph
is-an-author: 1
\\
  We identify an invariant light-front coordinate $\zeta$ which allows the
separation of the dynamics of quark and gluon binding from the kinematics of
constituent spin and internal orbital angular momentum. The result is a
single-variable light-front Schrodinger equation for QCD which determines the
eigenspectrum and the light-front wavefunctions of hadrons for general spin and
orbital angular momentum. This frame-independent light-front wave equation is
equivalent to the equations of motion which describe the propagation of
spin-$J$ modes on anti-de Sitter (AdS) space. Light-front holography is a
remarkable feature of AdS/CFT: it allows hadronic amplitudes in the AdS fifth
dimension to be mapped to frame-independent light-front wavefunctions of
hadrons in physical space-time, thus providing a relativistic description of
hadrons at the amplitude level. In principle, the model can be systematically
improved by diagonalizing the full QCD light-front Hamiltonian on the AdS/QCD
basis. Quark and gluon hadronization can be computed at the amplitude level by
convoluting the off-shell $T$ matrix calculated from the QCD light-front
Hamiltonian with the hadronic light-front wavefunctions. We also note the
distinction between static observables such as the probability distributions
computed from the square of the light-front wavefunctions versus dynamical
observables such as the structure functions and the leading-twist single-spin
asymmetries measured in deep inelastic scattering which include the effects of
initial and final-state interactions.
\\


#warnings_now: ADMIN UPLOAD



#author_warnings_now: 
Author 1: Stanley J. Brodsky
Author 2: Guy F. de Teramond
-> Number of authors = 2



#####Fri Oct 10 08:53:33 2008#####
Finished unpacking (errors=)

#author_warnings_now: 
Author 1: Stanley J. Brodsky
Author 2: Guy F. de Teramond
-> Number of authors = 2

 9999151.tar: unpacked 10 files from tar file
 hep-ph.gfdt.19143.tar: unpacked 5 files from tar file


#####Fri Oct 10 08:53:33 2008#####
showtime: 0810.1876 being processed as test/9999151 -> /data/ftp/arxiv/papers/0810


#####Fri Oct 10 08:53:33 2008#####
packing to 0810.1876.tar.gz

#####Fri Oct 10 08:53:33 2008#####
running AutoTeX -p test/9999151 -d 0810.1876 at Fri Oct 10 08:53:33 2008

#####Fri Oct 10 08:53:34 2008#####
completed AutoTeX in 1s

#####Fri Oct 10 08:53:34 2008#####
Rejected after unpack_submission()... cleaning up

#warnings_now: ADMIN UPLOAD

Fri Oct 10 08:53:34 2008: AutoTeX took 1s


#####Fri Oct 10 08:53:34 2008#####
About to close and move this log to /u0/incoming/admin_hep-ph.gfdt.19143 which will then be moved to /u0/incoming/rejects


==> debug_log_9717 <==

#####Fri Oct 10 08:46:56 2008#####
STARTED admin_hep-ph.gfdt.19143


#####Fri Oct 10 08:46:56 2008#####
------------------------------------------------------------------------------
\\
arXiv:0810.1873
From: Guy F. de T\'eramond <gdt@asterix.crnet.cr>
Date: Fri, 10 Oct 2008 02:45:58 GMT   (000kb)

Title: The AdS/CFT Correspondence and Light-Front QCD
Authors: Stanley J. Brodsky and Guy F. de Teramond
Categories: hep-ph
Comments: 12 pages, 4 figures. Presented by SJB at LIGHT CONE 2008:
  Relativistic Nuclear and Particle Physics
Report-no: SLAC-PUB-13428
License: http://arxiv.org/licenses/nonexclusive-distrib/1.0/
Policy: accept
Upload-archive: hep-ph
Upload-subject: hput admin_hep-ph.gfdt.19143 figscombine.pdf LFHolography.pdf
  StaticDynamic.pdf
archive: hep-ph
is-an-author: 1
\\
  We identify an invariant light-front coordinate $\zeta$ which allows the
separation of the dynamics of quark and gluon binding from the kinematics of
constituent spin and internal orbital angular momentum. The result is a
single-variable light-front Schrodinger equation for QCD which determines the
eigenspectrum and the light-front wavefunctions of hadrons for general spin and
orbital angular momentum. This frame-independent light-front wave equation is
equivalent to the equations of motion which describe the propagation of
spin-$J$ modes on anti-de Sitter (AdS) space. Light-front holography is a
remarkable feature of AdS/CFT: it allows hadronic amplitudes in the AdS fifth
dimension to be mapped to frame-independent light-front wavefunctions of
hadrons in physical space-time, thus providing a relativistic description of
hadrons at the amplitude level. In principle, the model can be systematically
improved by diagonalizing the full QCD light-front Hamiltonian on the AdS/QCD
basis. Quark and gluon hadronization can be computed at the amplitude level by
convoluting the off-shell $T$ matrix calculated from the QCD light-front
Hamiltonian with the hadronic light-front wavefunctions. We also note the
distinction between static observables such as the probability distributions
computed from the square of the light-front wavefunctions versus dynamical
observables such as the structure functions and the leading-twist single-spin
asymmetries measured in deep inelastic scattering which include the effects of
initial and final-state interactions.
\\


#warnings_now: ADMIN UPLOAD



#author_warnings_now: 
Author 1: Stanley J. Brodsky
Author 2: Guy F. de Teramond
-> Number of authors = 2



#####Fri Oct 10 08:46:56 2008#####
Finished unpacking (errors=)

#author_warnings_now: 
Author 1: Stanley J. Brodsky
Author 2: Guy F. de Teramond
-> Number of authors = 2

 hep-ph.gfdt.19143.tar: unpacked 5 files from tar file


#####Fri Oct 10 08:46:56 2008#####
showtime: 0810.1873 being processed as test/9999151 -> /data/ftp/arxiv/papers/0810


#####Fri Oct 10 08:46:56 2008#####
packing to 0810.1873.tar.gz

#####Fri Oct 10 08:46:56 2008#####
running AutoTeX -p test/9999151 -d 0810.1873 at Fri Oct 10 08:46:56 2008

#####Fri Oct 10 08:46:57 2008#####
completed AutoTeX in 1s

#####Fri Oct 10 08:46:57 2008#####
Rejected after unpack_submission()... cleaning up

#warnings_now: ADMIN UPLOAD

Fri Oct 10 08:46:57 2008: AutoTeX took 1s


#####Fri Oct 10 08:46:57 2008#####
About to close and move this log to /u0/incoming/admin_hep-ph.gfdt.19143 which will then be moved to /u0/incoming/rejects

